Opportunistic Synthesis in Reactive Games under Information Asymmetry

Reactive synthesis is a class of methods to construct a provably-correct control system, referred to as a robot, with respect to a temporal logic specification in the presence of a dynamic and uncontrollable environment. This is achieved by modeling the interaction between the robot and its environment as a two-player zero-sum game. However, existing reactive synthesis methods assume both players to have complete information, which is not the case in many strategic interactions. In this paper, we use a variant of hypergames to model the interaction between the robot and its environment; which has incomplete information about the specification of the robot. This model allows us to identify a subset of game states from where the robot can leverage the asymmetrical information to achieve a better outcome, which is not possible if both players have symmetrical and complete information. We then introduce a novel method of opportunistic synthesis by defining a Markov Decision Process (MDP) using the hypergame under temporal logic specifications. When the environment plays some stochastic strategy in its perceived sure-winning and sure-losing regions of the game, we show that by following the opportunistic strategy, the robot is ensured to only improve the outcome of the game - measured by satisfaction of sub-specifications - whenever an opportunity becomes available. We demonstrate the correctness and optimality of this method using a robot motion planning example in the presence of an adversary.

==> include/defs.tex <==
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% based on defs.tex by S. Boyd
% modified by Jie Fu
\newif\ifuseboldmathops
\newif\ifuseittextabbrevs
\useboldmathopstrue   % comment out to use mathbb
%\useittextabbrevstrue % comment out to use non-italic text abbrevs like e.g.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% text abbrevs
\ifuseittextabbrevs
	\newcommand{\cf}{{\it cf.}}
	\newcommand{\eg}{{\it e.g.}}
	\newcommand{\ie}{{\it i.e.}}
	\newcommand{\etc}{{\it etc.}}
	\newcommand{\etal}{{et~al.}}
\else
	\newcommand{\cf}{cf.}
	\newcommand{\eg}{e.g.}
	\newcommand{\ie}{i.e.}
	\newcommand{\etc}{etc.}
	\newcommand{\etal}{et~al.}
\fi

% standard math sets
\ifuseboldmathops
	%\newcommand{\reals}{{\mbox{\bf R}}}
	\newcommand{\reals}{\mathbf{R}}
	\newcommand{\integers}{\mathbf{Z}}
	\newcommand{\complex}{\mathbf{C}}
	\newcommand{\symm}{\mathbf{S}}  % symmetric matrices
\else
	\newcommand{\reals}{\mathbb{R}}
	\newcommand{\integers}{\mathbb{Z}}
	\newcommand{\complex}{\mathbb{C}}
	\newcommand{\symm}{\mathbb{S}}  % symmetric matrices
\fi

% control theory sets
\ifuseboldmathops
	\newcommand{\HH}{\mathbf{H}}
	\newcommand{\LL}{\mathbf{L}}
\else
	\newcommand{\HH}{\mathbb{H}}
	\newcommand{\LL}{\mathbb{L}}
\fi

% probability operators
\ifuseboldmathops
	\newcommand{\Expect}{\mathop{\bf E{}}\nolimits}
	\newcommand{\Prob}{\mathop{\bf P{}}\nolimits}
\else
	\newcommand{\Expect}{\mathop{\mathbb{E}{}}\nolimits}
	\newcommand{\Prob}{\mathop{\mathbb{P}{}}\nolimits}
\fi

% convex operators
\ifuseboldmathops
	\renewcommand{\Re}{\mathop{\bf Re}}
	\renewcommand{\Im}{\mathop{\bf Im}}
	
	\newcommand{\prox}{\mathop{\bf prox}} % proximal operator
	\newcommand{\dom}{\mathop{\bf dom}}   % domain
	\newcommand{\aff}{\mathop{\bf aff}}   % affine hull
	\newcommand{\cl}{\mathop{\bf cl}}     % closure
	\newcommand{\intr}{\mathop{\bf int}}  % interior
	\newcommand{\Co}{\mathop{\bf Co}}     % convex hull
	\newcommand{\relint}{\mathop{\bf rel int}} % relative interior
	\newcommand{\bd}{\mathop{\bf bd}}     % boundary
	
	\newcommand{\Tr}{\mathop{\bf Tr}}
	\newcommand{\diag}{\mathop{\bf diag}}
\else
	\renewcommand{\Re}{\mathop{\mathrm{Re}}}
	\renewcommand{\Im}{\mathop{\mathrm{Im}}}
	
	\newcommand{\prox}{\mathop{\mathrm{prox}}} % proximal operator
	\newcommand{\dom}{\mathop{\mathrm{dom}}}   % domain
	\newcommand{\aff}{\mathop{\mathrm{aff}}}   % affine hull
	\newcommand{\cl}{\mathop{\mathrm{cl}}}     % closure
	\newcommand{\intr}{\mathop{\mathrm{int}}}  % interior
	\newcommand{\Co}{\mathop{\mathrm{Co}}}     % convex hull
	\newcommand{\relint}{\mathop{\mathrm{rel int}}} % relative interior
	\newcommand{\bd}{\mathop{\mathrm{bd}}}     % boundary
	
	\newcommand{\Tr}{\mathop{\mathrm{Tr}}}     % trace
	\newcommand{\diag}{\mathop{\mathrm{diag}}} % diagonal matrix
\fi

% useful non-bold operators
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\eqbyset}{\mathrel{\stackrel{\mathrm{set}}{=}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}

% lin alg stuff
\newcommand{\Span}{\mathop{\mathrm{span}}}
\newcommand{\Range}{\mathop{\mathrm{range}}}
\newcommand{\Null}{\mathop{\mathrm{null}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}

\newcommand{\ones}{\mathbf 1}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{{\lambda_{\rm min}}}
\newcommand{\sigmamax}{{\sigma_{\rm max}}}
\newcommand{\sigmamin}{{\sigma_{\rm min}}}

% linear temporal logic 
% from Baier, Katoen
\newcommand{\Always}{\Box \, }
\newcommand{\Eventually}{\Diamond \, }
\newcommand{\Next}{\bigcirc \, }
\newcommand{\until}{\mbox{$\, {\sf U}\,$}}
\newcommand{\R}{\mbox{$\, {\sf R}\,$}}
\newcommand{\Unless}{\mbox{$\, {\sf W}\,$}}
\newcommand{\Model}{{\cal K}}
% \newcommand{\Eventually}{\mbox{$\tilde{{\sf F}} \, $}}
% \newcommand{\Untils}{\mbox{$\, \tilde{{\sf U}}\,$}}
% \newcommand{\Alwaysp}{\mbox{${\sf G}^{{-}1} \, $}}
% \newcommand{\Everp}{\mbox{${\sf F}^{{-}1} \, $}}
% \newcommand{\Nextp}{\mbox{${\sf X}^{{-}1} \, $}}


\newcommand{\G}{\Always}
\newcommand{\U}{\Until}
\newcommand{\WU}{\mbox{$\, {\sf W}\,$}}
\newcommand{\Release}{\mbox{$\, {\sf R}\,$}}
\newcommand{\X}{\Next}
%\newcommand{\V}{\mbox{$\, \overline{{\sf U}} \,$}}
\newcommand{\Lagrange}{\mathcal{L}}

%\newcommand{\Always}{\Box \, }
 %\newcommand{\Eventually}{\Diamond \, }
% \newcommand{\Next}{\bigcirc \, }
\newcommand{\sink}{\mathsf{sink} }

%\newcommand{\Next}{\kern0.5ex\vcenter{\hbox{$\scriptstyle\bigcirc$}}\kern0.5ex}
\newcommand{\BoolTrue}{\mbox{\sf true}}
\newcommand{\BoolFalse}{\mbox{\sf false}}
\newcommand{\agg}{\mathcal{A}}
\newcommand{\normal}[1]{\mathcal{N}\left(#1\right)}

\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\grid}[1]{\left[#1\right]}

\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\stateof}[1]{\llbracket#1\rrbracket}

\newcommand{\dist}[1]{\mbox{Dist}(#1)}
\newcommand{\prob}{\mbox{Prob}}

\newcommand{\supp}{\mbox{Supp}}


\newcommand{\labelcost}{\mbox{goal}}
\newcommand{\bigO}{\mathbb{O}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calL}{\mathcal{L}}

\newcommand{\fac}{\mathsf{fac}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calS}{\mathcal{S}}

\newcommand{\calAP}{\mathcal{AP}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calM}{\mathcal{M}}

\newcommand{\calG}{\mathcal{G}}



\newcommand{\init}{\mathsf{Init}}
\newcommand{\final}{\mathsf{Final}}
\newcommand{\suff}{\mathsf{Suff}}
\newcommand{\last}{\mathsf{Last}}
\newcommand{\semi}{\mathsf{semi}}


\newcommand{\guard}{\mathsf{Guard}}
\newcommand{\task}{\mathcal{T}}
\newcommand{\arena}{\mathsf{TS}}

\newcommand{\val}{\mathcal{V}}
\newcommand{\prog}{\mathsf{Prog}}



\newcommand{\reach}{\mathfrak{R}}

\newcommand{\avoid}{\mathfrak{O}}
\newcommand{\cost}{\mathcal{C}}
\newcommand{\softmax}{\mbox{softmax}}
\newcommand{\softmin}{\mbox{softmin}}

\newcommand{\softidx}{\mbox{softidx}}


\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\inside}[1]{\llbracket
{#1} \rrbracket
}

\newcommand{\idx}{\mathbf{\eta}}

\newcommand{\nat}{\mathbb{Z}}

\newcommand{\weight}{\mathbf{w}}
\newcommand{\prodInit}{\hat{\mu}} 
\newcommand{\prodP}{\hat{P}} 
\newcommand{\option}{\mathsf{O}} 


% acronym

\acrodef{mdp}[MDP]{Markov decision process}
\acrodef{gcd}[GCD]{Generalized Conjunction/Disjunction}
\acrodef{dfa}[DFA]{deterministic finite-state automaton}
\acrodef{ltl}[LTL]{linear temporal logic}
\acrodef{ag}[AG]{Assume-Guarantee}
\acrodef{ssp}[SSP]{Stochastic Shortest Path}

%%% define the theorem environment

\theoremstyle{definition}
 \newtheorem{definition}{Definition}
 \newtheorem{example}{Example}
\newtheorem{problem}{Problem}
\newtheorem{lemma}{Lemma}

\newcommand{\attr}{\mathsf{Attr}}



%%% define acronym
\acrodef{ltl}[LTL]{linear temporal logic formula}
\acrodef{mdp}[MDP]{Markov decision process}
\acrodef{smdp}[Semi-MDP]{Semi-Markov decision process}

\acrodef{scltl}[scLTL]{syntactically co-safe LTL}
